$\mathfrak{hs}$-extended gravity from the IKKT matrix model

We elaborate further on the one-loop effective action of the IKKT model on 3 + 1 dimensional covariant quantum spacetime in the presence of fuzzy extra dimensions. In particular, we describe the one-loop effective action in terms of a remarkable $SO(1, 9)$ character, which allows to evaluate the pertinent traces over the internal modes explicitly. This also allows to estimate the higher-order contributions (in the internal flux $\mathcal{F}_{\mathtt{IJ}}$) to the one-loop effective action in a systematic way. We show that all higher-order contributions are generally suppressed and UV finite, which justifies the previous treatment of the induced gravitational action. We also obtain explicit expressions for the effective Newton constant, and determine the dynamics of the Kaluza-Klein scale $\Delta_{\mathcal{K}}$ of the fuzzy extra dimensions $\mathcal{K}$.

==> YoungDiagrams.tex <==

\newcommand{\bep}{\begin{picture}}
\newcommand{\eep}{\end{picture}}

\newcommand{\smallpic}[1]{{\unitlength=0.2mm#1}}
\newcommand{\minorpic}[1]{{\unitlength=0.30mm#1}}
\newcommand{\boldpic}[1]{{\linethickness{0.4mm}#1}}
\newcommand{\smallboldpic}[1]{{\unitlength=0.2mm\linethickness{0.35mm}#1}}


% counters to make some coordinates calculations
\newcounter{Summa}
\newcounter{Inc}
\newcounter{Dec}

\newcounter{YoungHeight}\newcounter{YoungWidth}

\newcounter{Mul1}\newcounter{Mul2}\newcounter{Mul3}\newcounter{Mul4}
\newcounter{A0}\newcounter{A1}\newcounter{A2}\newcounter{A3}\newcounter{A4}\newcounter{A5}\newcounter{A6}
\newcounter{B0}\newcounter{B1}\newcounter{B2}\newcounter{B3}\newcounter{B4}\newcounter{B5}
\newcounter{C0}\newcounter{C1}\newcounter{C2}\newcounter{C3}\newcounter{C4}\newcounter{C5}\newcounter{C6}\newcounter{C7}\newcounter{C8}
\newcounter{D0}\newcounter{D1}\newcounter{D2}\newcounter{D3}\newcounter{D4}\newcounter{D5}
\newcounter{T0}\newcounter{T1}\newcounter{T2}\newcounter{T3}\newcounter{T4}\newcounter{T5}

\newlength{\txtVShift}
\newlength{\txtHShift}
\newlength{\txtHeight}
\newlength{\txtWidth}

% multimplications by 5 and by 10
\newcommand{\HalfLength}[2]{\setcounter{Mul1}{#1}\setcounter{Mul2}{#1}\addtocounter{Mul1}{\value{Mul2}}\addtocounter{Mul1}{\value{Mul2}}%
\addtocounter{Mul1}{\value{Mul2}}\addtocounter{Mul1}{\value{Mul2}}\setcounter{#2}{\value{Mul1}}}
\newcommand{\HalfLengthB}[2]{\setcounter{Mul3}{#1}\setcounter{Mul4}{#1}\addtocounter{Mul3}{\value{Mul4}}\addtocounter{Mul3}{\value{Mul4}}%
\addtocounter{Mul3}{\value{Mul4}}\addtocounter{Mul3}{\value{Mul4}}\setcounter{#2}{\value{Mul3}}}
\newcommand{\MulTen}[2]{\HalfLength{#1}{#2}\addtocounter{#2}{\value{#2}}}

% fast Add/Sub operations  #1-counter name #2-init value #3 - value to be added
\newcommand{\Inc}[2]{\setcounter{#1}{#2}\addtocounter{#1}{1}}
\newcommand{\Dec}[2]{\setcounter{#1}{#2}\addtocounter{#1}{-1}}
\newcommand{\Add}[3]{\setcounter{#1}{#2}\addtocounter{#1}{#3}}
\newcommand{\Sub}[3]{\setcounter{#1}{#2}\addtocounter{#1}{-#3}}

% box to size unit and scales, other constants
\newcommand{\Length}[1]{#10}
\newcommand{\PictureScale}{}%\unitlength=0.25mm}
\newcommand{\YoungScale}{}%\unitlength=0.35mm}
\newcommand{\SmoothLength}{14}
\newcommand{\SmoothTip}{4}



%commands to place text in different areas of rectangular region
\newcommand{\shiftedText}[2]{{\hspace{#1}#2}}
\newcommand{\calcHShift}[1]{\settowidth{\txtWidth}{#1}\setlength{\txtHShift}{-0.5\txtWidth}}
\newcommand{\calcHShiftFull}[1]{\settowidth{\txtWidth}{#1}\setlength{\txtHShift}{-1.0\txtWidth}}

\newcommand{\TextCenter}[3]{{\HalfLength{#2}{T0}%
\HalfLength{#3}{T1}\addtocounter{T1}{-3}\calcHShift{#1}%
\put(\value{T0},\value{T1}){\shiftedText{\txtHShift}{#1}}}}
\newcommand{\TextCenterShiftX}[4]{{\HalfLength{#3}{T0}\addtocounter{T0}{#2}%
\HalfLength{#4}{T1}\addtocounter{T1}{-3}\calcHShift{#1}%
\put(\value{T0},\value{T1}){\shiftedText{\txtHShift}{#1}}}}
\newcommand{\TextCenterA}[3]{{\HalfLength{#2}{T0}%
\HalfLength{#3}{T1}\addtocounter{T1}{-3}\addtocounter{T0}{10}\calcHShift{#1}%
\put(\value{T0},\value{T1}){\shiftedText{\txtHShift}{#1}}}}
\newcommand{\TextCenterB}[3]{{\calcHShift{#1}\HalfLength{#2}{T0}\Add{T1}{\Length{#3}}{-7}\put(\value{T0},\value{T1}){\shiftedText{\txtHShift}{#1}}}}
\newcommand{\TextCenterShift}[4]{{\HalfLength{#3}{T0}\addtocounter{T0}{-3}\HalfLength{#4}{T1}\addtocounter{T1}{#2}\put(\value{T0},\value{T1}){#1}}}
%\newcommand{\TextCenter}[3]{{\calcHShift{#1}\HalfLength{#2}{T0}\Add{T1}{\Length{#3}}{-9}\put(\value{T0},\value{T1}){\shiftedText{\txtHShift}{#1}}}}
\newcommand{\TextBottom}[3]{{\HalfLength{#2}{T0}\addtocounter{T0}{-5}\put(\value{T0},2){#1}}}
\newcommand{\TextOver}[3]{{\HalfLength{#2}{T0}\addtocounter{T0}{-3}\Add{T1}{\Length{#3}}{1}\put(\value{T0},\value{T1}){#1}}}
\newcommand{\TextUnder}[3]{{\HalfLength{#2}{T0}\addtocounter{T0}{-5}\put(\value{T0},-9){#1}}}
\newcommand{\TextUnderA}[3]{{\HalfLength{#2}{T0}\calcHShift{#1}\put(\value{T0},-7){\shiftedText{\txtHShift}{$\scriptstyle #1$}}}}
\newcommand{\TextUnderB}[3]{{\HalfLength{#2}{T0}\calcHShiftA{#1}\put(\value{T0},-7){\shiftedText{\txtHShift}{$\scriptstyle #1$}}}}\newcommand{\TextRightIn}[3]{{\HalfLength{#3}{T1}\addtocounter{T1}{-5}\Add{T0}{\Length{#2}}{0}\calcHShiftFull{#1}%
\put(\value{T0},\value{T1}){\shiftedText{\txtHShift}{#1}}}}
\newcommand{\TextLeftIn}[3]{{\HalfLength{#3}{T1}\addtocounter{T1}{-5}\put(2,\value{T1}){#1}}}
\newcommand{\TextLeft}[3]{{\HalfLength{#3}{T1}\addtocounter{T1}{-5}\calcHShiftFull{#1}\put(0,\value{T1}){\shiftedText{\txtHShift}{#1}}}}
\newcommand{\TextRight}[3]{{\HalfLength{#3}{T1}\addtocounter{T1}{-5}\Add{T0}{\Length{#2}}{2}\put(\value{T0},\value{T1}){#1}}}
\newcommand{\TextRightTop}[3]{{\Add{T1}{\Length{#3}}{-9}\Add{T0}{\Length{#2}}{2}\put(\value{T0},\value{T1}){#1}}}
\newcommand{\TextRightT}[3]{{\HalfLength{#3}{T1}\addtocounter{T1}{1}\Add{T0}{\Length{#2}}{2}\put(\value{T0},\value{T1}){#1}}}
\newcommand{\TextTopRight}[4]{{\TextTop{#1}{#3}{#4}\TextRight{#2}{#3}{#4}}}
\newcommand{\TextTopRightIn}[4]{{\TextTop{#1}{#3}{#4}\TextRightIn{#2}{#3}{#4}}}
\newcommand{\TextTopLeftIn}[4]{{\TextTop{#1}{#3}{#4}\TextLeftIn{#2}{#3}{#4}}}
\newcommand{\TextBottomRight}[4]{{\TextBottom{#1}{#3}{#4}\TextRight{#2}{#3}{#4}}}
\newcommand{\TextTopRightT}[4]{{\TextTop{#1}{#3}{#4}\TextRightT{#2}{#3}{#4}}}
\newcommand{\TextBottomRightT}[4]{{\TextBottom{#1}{#3}{#4}\TextRightT{#2}{#3}{#4}}}




% Main commands to create Blocks
\newcommand{\BlockA}[2]{{\YoungScale\bep(\Length{#1},\Length{#2}){\Add{A1}{#1}{1}\Add{A2}{#2}{1}}%
\multiput(0,0)(10,0){\value{A1}}{\line(0,1){\Length{#2}}}\multiput(0,0)(0,10){\value{A2}}{\line(1,0){\Length{#1}}}%
\setcounter{YoungHeight}{\Length{#2}}\setcounter{YoungWidth}{\Length{#1}}\eep}}

\newcommand{\BlockB}[4]{{\YoungScale\Add{B3}{\Length{#2}}{\Length{#4}}%
\bep(\Length{#1},\value{B3})\put(0,\Length{#4}){\BlockA{#1}{#2}}%
\put(0,0){\BlockA{#3}{#4}}\setcounter{YoungHeight}{\value{B3}}\setcounter{YoungWidth}{\Length{#1}}\eep}}

\newcommand{\BlockC}[6]{{\YoungScale\Add{C3}{\Length{#4}}{\Length{#6}}\Add{C4}{\value{C3}}{\Length{#2}}%
\bep(\Length{#1},\value{C4})\put(0,\value{C3}){\BlockA{#1}{#2}}\put(0,\Length{#6}){\BlockA{#3}{#4}}%
\put(0,0){\BlockA{#5}{#6}}\setcounter{YoungHeight}{\value{C4}}\setcounter{YoungWidth}{\Length{#1}}\eep}}

\newcommand{\BlockD}[8]{{\YoungScale\Add{D1}{\Length{#8}}{\Length{#6}}\Add{D2}{\value{D1}}{\Length{#4}}\Add{D3}{\value{D2}}{\Length{#2}}%
\bep(\Length{#1},\value{D3})\put(0,\value{D2}){\BlockA{#1}{#2}}\put(0,0){\BlockC{#3}{#4}{#5}{#6}{#7}{#8}}%
\setcounter{YoungHeight}{\value{D3}}\setcounter{YoungWidth}{\Length{#1}}\eep}}




% Block with text defined by #3, which is a full command
\newcommand{\RectT}[3]{\bep(\Length{#1},\Length{#2})\put(0,0){\line(1,0){\Length{#1}}}\put(0,0){\line(0,1){\Length{#2}}}%
\put(\Length{#1},\Length{#2}){\line(-1,0){\Length{#1}}}\put(\Length{#1},\Length{#2}){\line(0,-1){\Length{#2}}}#3{#1}{#2}\eep}



% one, two and three rows diagrams with text at each block
\newcommand{\RectARow}[2]{{\bep(\Length{#1},10)\put(0,0){\RectT{#1}{1}{\TextCenter{#2}}}\eep}}

\newcommand{\RectARowBlock}[3]{{\bep(0,0)#3\eep\Add{A0}{\value{YoungHeight}}{10}\bep(\Length{#1},\value{A0})%
\put(0,\value{YoungHeight}){\RectT{#1}{1}{\TextCenter{#2}}}\eep}}

\newcommand{\RectBRow}[4]{{\bep(\Length{#1},20)\put(0,0){\RectT{#2}{1}{\TextBottom{#4}}}%
\put(0,10){\RectT{#1}{1}{\TextBottom{#3}}}\eep}}

\newcommand{\RectCRow}[6]{{\bep(\Length{#1},30)\put(0,0){\RectT{#3}{1}{\TextCenter{#6}}}%
\put(0,10){\RectT{#2}{1}{\TextCenter{#5}}}\put(0,20){\RectT{#1}{1}{\TextCenter{#4}}}\eep}}

\newcommand{\RectARowUp}[2]{{\bep(\Length{#1},10)\put(0,0){\RectT{#1}{1}{\TextCenter{#2}}}\eep}}

\newcommand{\RectBRowUp}[4]{{\bep(\Length{#1},20)\put(0,0){\RectT{#2}{1}{\TextCenter{#4}}}%
\put(0,10){\RectT{#1}{1}{\TextCenter{#3}}}\eep}}

\newcommand{\RectCRowUp}[6]{{\bep(\Length{#1},30)\put(0,0){\RectT{#3}{1}{\TextCenterB{#6}}}%
\put(0,10){\RectT{#2}{1}{\TextCenterB{#5}}}\put(0,20){\RectT{#1}{1}{\TextCenterB{#4}}}\eep}}

% diagram with one row at the right
\newcommand{\RectAYoung}[3]{{\bep(0,0)#3\eep\Add{A0}{\value{YoungWidth}}{\Length{#1}}%
\Add{A1}{\value{YoungHeight}}{-10}\bep(\value{A0},\value{YoungHeight})%
\put(\value{YoungWidth},\value{A1}){\RectT{#1}{1}{\TextCenter{#2}}}\eep}}

\newcommand{\RectBYoung}[3]{{\bep(0,0)\put(0,0){#3}\eep\Add{A0}{\value{YoungHeight}}{10}%
\bep(\Length{#1},\value{A0})%
\put(0,\value{YoungHeight}){\RectT{#1}{1}{\TextCenter{#2}}}\eep}}

\newcommand{\RectCYoung}[5]{{\bep(0,0)\put(0,0){#5}\eep\Add{A0}{\value{YoungHeight}}{20}%
\bep(\Length{#1},\value{A0})%
\put(0,\value{YoungHeight}){\RectBRow{#1}{#2}{#3}{#4}}\eep}}

\newcommand{\RectDYoung}[7]{{\bep(0,0)\put(0,0){#7}\eep\Add{A0}{\value{YoungHeight}}{30}%
\bep(\Length{#1},\value{A0})%
\put(0,\value{YoungHeight}){\RectCRow{#1}{#2}{#3}{#4}{#5}{#6}}\eep}}




\newcommand{\Rectangle}[2]{\bep(#1,#2)\put(0,0){\line(1,0){#1}}\put(0,0){\line(0,1){#2}}%
\put(#1,#2){\line(-1,0){#1}}\put(#1,#2){\line(0,-1){#2}}\eep}



\newcommand{\YoungA}{\BlockA{1}{1}}
\newcommand{\YoungB}{\BlockA{2}{1}}
\newcommand{\YoungC}{\BlockA{3}{1}}
\newcommand{\YoungD}{\BlockA{4}{1}}
\newcommand{\YoungE}{\BlockA{5}{1}}
\newcommand{\YoungF}{\BlockA{6}{1}}

\newcommand{\YoungAA}{\BlockA{1}{2}}
\newcommand{\YoungBA}{\BlockB{2}{1}{1}{1}}
\newcommand{\YoungBB}{\BlockA{2}{2}}
\newcommand{\YoungCA}{\BlockB{3}{1}{1}{1}}
\newcommand{\YoungCB}{\BlockB{3}{1}{2}{1}}
\newcommand{\YoungCC}{\BlockA{3}{2}}
\newcommand{\YoungDA}{\BlockB{4}{1}{1}{1}}
\newcommand{\YoungDB}{\BlockB{4}{1}{2}{1}}
\newcommand{\YoungDC}{\BlockB{4}{1}{3}{1}}
\newcommand{\YoungDD}{\BlockA{4}{2}}

\newcommand{\YoungAAA}{\BlockA{1}{3}}
\newcommand{\YoungBAA}{\BlockB{2}{1}{1}{2}}
\newcommand{\YoungBBA}{\BlockB{2}{2}{1}{1}}
\newcommand{\YoungBBB}{\BlockA{2}{3}}
\newcommand{\YoungCAA}{\BlockB{3}{1}{1}{2}}
\newcommand{\YoungCBA}{\BlockC{3}{1}{2}{1}{1}{1}}
\newcommand{\YoungCCA}{\BlockB{3}{2}{1}{1}}
\newcommand{\YoungCBB}{\BlockB{3}{1}{2}{2}}
\newcommand{\YoungCCB}{\BlockB{3}{2}{2}{1}}
\newcommand{\YoungCCC}{\BlockA{3}{3}}
\newcommand{\YoungDAA}{\BlockB{4}{1}{1}{2}}
\newcommand{\YoungDBA}{\BlockC{4}{1}{2}{1}{1}{1}}
\newcommand{\YoungDCA}{\BlockC{4}{1}{3}{1}{1}{1}}
\newcommand{\YoungDCB}{\BlockC{4}{1}{3}{1}{2}{1}}
\newcommand{\YoungDDA}{\BlockB{4}{2}{1}{1}}
\newcommand{\YoungAAAA}{\BlockA{1}{4}}
\newcommand{\YoungBAAA}{\BlockB{2}{1}{1}{3}}
\newcommand{\YoungBBAA}{\BlockB{2}{2}{1}{2}}
\newcommand{\YoungCCAA}{\BlockB{3}{2}{1}{2}}
\newcommand{\YoungCAAA}{\BlockB{3}{1}{1}{3}}

\newcommand{\YoungAAAAAA}{\BlockA{1}{6}}
\newcommand{\YoungBBBB}{\BlockA{2}{4}}
\newcommand{\YoungBAAAA}{\BlockB{2}{1}{1}{4}}

\newcommand{\Youngfourrow}{\BlockB{4}{1}{0}{0}}
% Main commands to create Blocks
\newcommand{\BlockApar}[2]{\parbox{\Length{#1}pt}{\YoungScale\bep(\Length{#1},\Length{#2}){\Add{A1}{#1}{1}\Add{A2}{#2}{1}}%
\multiput(0,0)(10,0){\value{A1}}{\line(0,1){\Length{#2}}}\multiput(0,0)(0,10){\value{A2}}{\line(1,0){\Length{#1}}}%
\setcounter{YoungHeight}{\Length{#2}}\setcounter{YoungWidth}{\Length{#1}}\eep}}

\newcommand{\BlockBpar}[4]{\parbox{\Length{#1}pt}{\YoungScale\Add{B3}{\Length{#2}}{\Length{#4}}%
\bep(\Length{#1},\value{B3})\put(0,\Length{#4}){\BlockA{#1}{#2}}%
\put(0,0){\BlockA{#3}{#4}}\setcounter{YoungHeight}{\value{B3}}\setcounter{YoungWidth}{\Length{#1}}\eep}}

\newcommand{\BlockCpar}[6]{\parbox{\Length{#1}pt}{\YoungScale\Add{C3}{\Length{#4}}{\Length{#6}}\Add{C4}{\value{C3}}{\Length{#2}}%
\bep(\Length{#1},\value{C4})\put(0,\value{C3}){\BlockA{#1}{#2}}\put(0,\Length{#6}){\BlockA{#3}{#4}}%
\put(0,0){\BlockA{#5}{#6}}\setcounter{YoungHeight}{\value{C4}}\setcounter{YoungWidth}{\Length{#1}}\eep}}


\newcommand{\YoungpA}{\BlockApar{1}{1}}
\newcommand{\YoungpB}{\BlockApar{2}{1}}
\newcommand{\YoungpC}{\BlockApar{3}{1}}
\newcommand{\YoungpD}{\BlockApar{4}{1}}
\newcommand{\YoungpE}{\BlockApar{5}{1}}
\newcommand{\YoungpF}{\BlockApar{6}{1}}

\newcommand{\YoungpAA}{\BlockApar{1}{2}}
\newcommand{\YoungpBA}{\BlockBpar{2}{1}{1}{1}}
\newcommand{\YoungpBB}{\BlockApar{2}{2}}
\newcommand{\YoungpCA}{\BlockBpar{3}{1}{1}{1}}
\newcommand{\YoungpCB}{\BlockBpar{3}{1}{2}{1}}
\newcommand{\YoungpCC}{\BlockApar{3}{2}}
\newcommand{\YoungpDA}{\BlockBpar{4}{1}{1}{1}}
\newcommand{\YoungpDB}{\BlockBpar{4}{1}{2}{1}}
\newcommand{\YoungpDC}{\BlockBpar{4}{1}{3}{1}}
\newcommand{\YoungpDD}{\BlockApar{4}{2}}

\newcommand{\YoungpAAA}{\BlockApar{1}{3}}
\newcommand{\YoungpBAA}{\BlockBpar{2}{1}{1}{2}}
\newcommand{\YoungpBBA}{\BlockBpar{2}{2}{1}{1}}
\newcommand{\YoungpBBB}{\BlockApar{2}{3}}
\newcommand{\YoungpCAA}{\BlockBpar{3}{1}{1}{2}}
\newcommand{\YoungpCBA}{\BlockCpar{3}{1}{2}{1}{1}{1}}
\newcommand{\YoungpCCA}{\BlockBpar{3}{2}{1}{1}}
\newcommand{\YoungpCBB}{\BlockBpar{3}{1}{2}{2}}
\newcommand{\YoungpCCB}{\BlockBpar{3}{2}{2}{1}}
\newcommand{\YoungpCCC}{\BlockApar{3}{3}}
\newcommand{\YoungpDAA}{\BlockBpar{4}{1}{1}{2}}
\newcommand{\YoungpDBA}{\BlockCpar{4}{1}{2}{1}{1}{1}}
\newcommand{\YoungpDCA}{\BlockCpar{4}{1}{3}{1}{1}{1}}
\newcommand{\YoungpDCB}{\BlockCpar{4}{1}{3}{1}{2}{1}}
\newcommand{\YoungpDDA}{\BlockApar{4}{2}{1}{1}}
\newcommand{\YoungpAAAA}{\BlockApar{1}{4}}
\newcommand{\YoungpBAAA}{\BlockBpar{2}{1}{1}{3}}
\newcommand{\YoungpBBAA}{\BlockBpar{2}{2}{1}{2}}
\newcommand{\YoungpCCAA}{\BlockBpar{3}{2}{1}{2}}
\newcommand{\YoungpCAAA}{\BlockBpar{3}{1}{1}{3}}

\newcommand{\YoungpAAAAA}{\BlockApar{1}{5}}
\newcommand{\YoungpAAAAAA}{\BlockApar{1}{6}}

\newcommand{\BlockAm}[2]{\mbox{\smallpic{\YoungScale\bep(\Length{#1},\Length{#2}){\Add{A1}{#1}{1}\Add{A2}{#2}{1}}%
\multiput(0,0)(10,0){\value{A1}}{\line(0,1){\Length{#2}}}\multiput(0,0)(0,10){\value{A2}}{\line(1,0){\Length{#1}}}%
\setcounter{YoungHeight}{\Length{#2}}\setcounter{YoungWidth}{\Length{#1}}\eep}}}

\newcommand{\BlockBm}[4]{\mbox{\smallpic{\YoungScale\Add{B3}{\Length{#2}}{\Length{#4}}%
\bep(\Length{#1},\value{B3})\put(0,\Length{#4}){\BlockA{#1}{#2}}%
\put(0,0){\BlockA{#3}{#4}}\setcounter{YoungHeight}{\value{B3}}\setcounter{YoungWidth}{\Length{#1}}\eep}}}

\newcommand{\BlockCm}[6]{\mbox{\smallpic{\YoungScale\Add{C3}{\Length{#4}}{\Length{#6}}\Add{C4}{\value{C3}}{\Length{#2}}%
\bep(\Length{#1},\value{C4})\put(0,\value{C3}){\BlockA{#1}{#2}}\put(0,\Length{#6}){\BlockA{#3}{#4}}%
\put(0,0){\BlockA{#5}{#6}}\setcounter{YoungHeight}{\value{C4}}\setcounter{YoungWidth}{\Length{#1}}\eep}}}

\newcommand{\YoungmA}{\BlockAm{1}{1}}
\newcommand{\YoungmB}{\BlockAm{2}{1}}
\newcommand{\YoungmC}{\BlockAm{3}{1}}
\newcommand{\YoungmD}{\BlockAm{4}{1}}
\newcommand{\YoungmE}{\BlockAm{5}{1}}
\newcommand{\YoungmF}{\BlockAm{6}{1}}

\newcommand{\YoungmAA}{\raisebox{-2pt}{\BlockAm{1}{2}}}
\newcommand{\YoungmBA}{\raisebox{-2pt}{\BlockBm{2}{1}{1}{1}}}
\newcommand{\YoungmBB}{\raisebox{-2pt}{\BlockAm{2}{2}}}
\newcommand{\YoungmCA}{\raisebox{-2pt}{\BlockBm{3}{1}{1}{1}}}
\newcommand{\YoungmCB}{\raisebox{-2pt}{\BlockBm{3}{1}{2}{1}}}
\newcommand{\YoungmCC}{\raisebox{-2pt}{\BlockAm{3}{2}}}
\newcommand{\YoungmDA}{\raisebox{-2pt}{\BlockBm{4}{1}{1}{1}}}
\newcommand{\YoungmDB}{\raisebox{-2pt}{\BlockBm{4}{1}{2}{1}}}
\newcommand{\YoungmDC}{\raisebox{-2pt}{\BlockBm{4}{1}{3}{1}}}
\newcommand{\YoungmDD}{\raisebox{-2pt}{\BlockAm{4}{2}}}


